GAPO: Learning Preferential Prompt through Generative Adversarial Policy Optimization

Recent advances in large language models have highlighted the critical need for precise control over model outputs through predefined constraints. While existing methods attempt to achieve this through either direct instruction-response synthesis or preferential response optimization, they often struggle with constraint understanding and adaptation. This limitation becomes particularly evident when handling fine-grained constraints, leading to either hallucination or brittle performance. We introduce Generative Adversarial Policy Optimization (GAPO), a novel framework that combines GAN-based training dynamics with an encoder-only reward model to progressively learn and adapt to increasingly complex constraints. GAPO leverages adversarial training to automatically generate training samples of varying difficulty while utilizing the encoder-only architecture to better capture prompt-response relationships. Extensive experiments demonstrate GAPO's superior performance across multiple benchmarks, particularly in scenarios requiring fine-grained constraint handling, where it significantly outperforms existing methods like PPO, DPO, and KTO. Our results suggest that GAPO's unique approach to preferential prompt learning offers a more robust and effective solution for controlling LLM outputs. Code is avaliable in https://github.com/MikeGu721/GAPO.

==> latex/01.Introduction.02.tex <==

With the rapid advancement of large language models (LLMs), there is an increasing demand for these models to generate content that satisfies specific constraints. As LLMs become more powerful, the need to guide their output to meet certain requirements—whether in terms of format, style, or content accuracy—becomes more pressing. This is particularly important in applications where adherence to constraints is essential, such as legal document generation, medical records, or content moderation.

Ensuring that language models can handle constraints during text generation is crucial. 
One effective approach to this is to control constraints at the data level. 
Data-level control can generally be achieved through two main types of synthetic data generation.
The first type directly synthesizes instruction-response pairs that satisfy the constraints, providing clear examples of compliant responses. 
The second type, which is often more effective, uses preference data to adjust the probability distribution, enhancing the likelihood that the model outputs a correct response over an incorrect one.

The first approach, although useful, often leads to “hallucination” problems, where the model generates content that diverges from the intended constraints. This limitation makes the second method—preference-based data synthesis—more widely used. A straightforward way to achieve preference-based data synthesis is to create pairs where prompts have been deliberately altered to produce responses that are either aligned or misaligned with constraints, providing the model with comparative examples. This method is simple, easy to implement, and supports fine-grained contrastive learning between correct and incorrect responses.

While this straightforward method offers utility, it often struggles to address more complex constraints, especially in decoder-only models. Due to their unidirectional attention mechanism, decoder-only models have difficulty recognizing mismatches between prompt and response. To enable more accurate understanding, we propose using an encoder-only model. With its bidirectional attention, an encoder-only model is well-suited to comprehending two-way dependencies in text and can more effectively discern inappropriate prompts for specific responses.

To refine this process further, we utilize Proximal Policy Optimization (PPO), which efficiently uses rewards from the encoder-only model’s discriminator to train the generator. The encoder-only model acts as a discriminator, assessing response compliance with constraints. Additionally, we employ a Generative Adversarial Network (GAN) to enhance this setup. In the GAN framework, the generator produces responses while the discriminator iteratively strengthens its ability to identify constraint violations by leveraging feedback from the generator’s current outputs. This iterative “enhancement” of the discriminator is essential, as it progressively sharpens the model’s capacity to detect nuanced violations, leading to more reliable constraint-aware responses.

==> latex/01.Introduction.03.tex <==


\begin{figure}
\centering
\includegraphics[width=\linewidth]{figs/intro.png}
\caption{
Illustration of the procedural differences between Supervised Fine-Tuning (SFT), Preferential Response Optimization, and Preferential Prompt Optimization, with emphasis on their distinct utilization of prompts and responses.
}
\label{fig:intro}
\end{figure}

The advent of large-scale models has induced significant transformations in practical applications, enabling models to comprehend a broad spectrum of human instructions, ranging from casual dialogue to intricate problem-solving tasks. As large language models (LLMs) advance in capability, the necessity for guiding their outputs to fulfill specific requirements—whether concerning format, style, or content accuracy—becomes increasingly critical. This is particularly vital in domains where compliance with constraints is paramount, such as legal document generation, medical record processing, and workflow automation.

Ensuring that language models adhere to predefined constraints during text generation is essential. One effective strategy for achieving this is training models to generate responses within specified boundaries at the data level. Data-level control is typically realized through two primary methods. The first method involves directly synthesizing instruction-response pairs that satisfy the constraints, offering clear examples of compliant outputs. The second method leverages preferential response data to adjust the probability distribution, thereby increasing the likelihood that the model produces an expected response rather than an unexpected one.

While the first approach can be effective, it often leads to the phenomenon of ``hallucination'', where the model, having learned only what constitutes a correct response, may resort to shortcuts that result in inaccurate or fabricated outputs. The second method is more commonly employed, as preferential response data allows the model to more precisely align its output with the desired response based on specific prompts. 
However, this approach does not necessarily enhance the model's understanding of the constraints embedded within the prompt. 
As illustrated in Figure~\ref{fig:intro}, modifying the constraints within the prompt is a straightforward task that can deepen the model’s comprehension of those constraints.

Although the direct modification method is straightforward, it presents challenges for decoder-only models, which are the dominant architecture in mainstream LLMs. Due to their unidirectional attention mechanism, decoder-only models encounter difficulties in detecting discrepancies between the prompt based on given response. In contrast, encoder-only models, with their bidirectional attention mechanism, are better suited to capture two-way dependencies in text. This allows encoder-only models to more effectively identify mismatches between the prompt and the response, thereby improving their ability to adhere to the constraints embedded within the prompt.

To better utilize preferential prompt data, we introduces the Generative Adversarial Policy Optimization (GAPO) algorithm in this paper. As the name suggests, the algorithm leverages a Generative Adversarial Network (GAN) to iteratively train a Reward Model, with the Proximal Policy Optimization (PPO) strategy used to update the generator. During the cold-start phase, the algorithm employs an encoder-only Reward Model to specifically learn the correspondence between prompts and responses, which is used to guide the training of the generator. In the adversarial training process, the Reward Model and generator engage in a competitive enhancement. The Reward Model treats the given prompt and the generator's response as mismatched, continuously generating reject prompts as negative samples based on the existing prompt-response data, while considering the original data as positive samples. Meanwhile, the generator strives to produce responses that deceive the Reward Model.

The advantages of GAPO are summarized as follows:
1. The use of an encoder-only Reward Model in GAPO effectively enhances the exploitation of preferential prompt data, enabling the language model to develop a deeper understanding of the intricate details within the prompt.
2. GAPO significantly simplifies the training process of the Reward Model in PPO. Traditionally, the performance of the Reward Model needed to be ensured before training an effective generator in PPO. In contrast, within the GAPO framework, the Reward Model and generator undergo iterative automated training, greatly reducing the complexity of Reward Model training.
3. According to our experiments, GAPO outperforms other baseline training methods, like PPO, DPO, KTO, ORPO, in learning from preferential prompt data. It also demonstrates superior performance in learning from general preferential response data. Thus, GAPO can be considered a more effective approach for enabling models to learn from preference data.

==> latex/02.RelatedWork.01.tex <==
\subsection{Reinforcement Learning with Human Feedback}

Reinforcement Learning from Human Feedback (RLHF)~\cite{bai2022rlhf, christiano2017deep, ziegler2019fine} aims at aligning LLMs with human values and expectations.
This approach enhances model outputs by utilizing human feedback to optimize the LLM's behavior.
Classical RLHF algorithms, such as Proximal Policy Optimization (PPO)~\cite{schulman2017ppo} and Direct Preference Optimization (DPO)~\cite{rafailov2024dpo}, exemplify this strategy.
PPO is widely employed due to its ability to maintain stability during training by employing a specialized reward model for evaluation~\cite{williams1992reinforce}.
In contrast, DPO, along with its derivatives such as SimPO~\cite{meng2024simpo}, IPO~\cite{azar2024ipo}, and KTO~\cite{ethayarajh2024kto}, streamlines the process by directly optimizing human preferences, thereby eliminating the need for a separate reward model and reducing computational complexity and bias~\cite{zheng2024balancing}.
Despite these advantages, RLHF generally demands substantial-high-quality feedback data, necessitating detailed labeling~\cite{bai2022rlhf}.
Moreover, DPO training is prone to overfitting, resulting in poor generalization to novel data~\cite{hu2024openrlhf}.



\subsection{Constraint Following Augmentation}

Prior work in constrained text generation can be broadly categorized into three main approaches~\cite{DBLP:journals/corr/abs-2201-05337}. The first category encompasses search-based methods, such as Constrained Beam Search (CBS)~\cite{anderson-etal-2017-guided} and its variants like Grid Beam Search (GBS)~\cite{hokamp-liu-2017-lexically} and Dynamic Beam Allocation (DBA)~\cite{post-vilar-2018-fast}, which enforce lexical constraints by modifying the search space, though often at the cost of generation speed and quality. The second category consists of score-based sampling methods that transform constraints into differentiable score functions~\cite{liu-etal-2022-dont}, offering greater flexibility in handling diverse constraint types but lacking guaranteed constraint satisfaction and suffering from slower generation speeds~\cite{qin2022cold}. The third category focuses on model-centric approaches, including specialized training methods and large language models like CTRL~\cite{keskar2019ctrl} and InstructCTG~\cite{DBLP:journals/corr/abs-2304-14293}, which incorporate constraints through pre-training or natural language instructions. Recent advancements have explored multiple directions: multi-attribute controlled text generation through prefix tuning~\cite{li2021prefix}; latent space manipulation techniques such as MacLaSa~\cite{ding-etal-2023-maclasa} and MAGIC~\cite{liu-etal-2024-multi}, where the latter employs counterfactual feature vectors to disentangle attributes; regular expression-based constraint generation through REI~\cite{zheng2023toward}; and the development of specialized datasets~\cite{zhang-etal-2023-macsum} to improve control ability while maintaining text quality.

% \citet{huang-etal-2023-extensible} have improved MACTG in prefix tuning\cite{li2021prefix} by adjusting the positions where prefixes are added, thereby reducing the mutual influence of multiple prefixes. Tailor~\cite{yang-etal-2023-tailor} adjust the multi-attribute prompt mask and re-index the position sequence to bridge the gap between the training phase (where each task uses a single-attribute prompt) and the testing phase (where two prompts are connected). 


% On the other hand, \citet{gu-etal-2022-distributional} approaches this issue from the perspective of distribution within semantic space. After obtaining the intersection of attribute distributions, the language model's distribution is biased toward this region. However, the intersection of different attribute distributions may not overlap. To address this, MacLaSa~\cite{ding-etal-2023-maclasa} estimates a compact latent space to improve control ability and text quality, mitigating interference between different aspects. \citet{liu-etal-2024-multi} propose MAGIC, which uses counterfactual feature vectors in the latent space to disentangle attributes, alleviating the imbalance in attribute correlation during training.
% REI~\cite{zheng2023toward} propose to use regular expression to facilitate constraint generation.

% Regarding the scarcity of training data for MCTG, \citet{zhang-etal-2023-macsum} propose MACSUM, a human-annotated dataset containing summaries with mixed control attributes. \citet{chen-etal-2023-mixture} use a strategy of mixing soft prompts to help large models generate training data that aligns with multi-aspect control attributes.

% Current approach for controllable text generation can be summarized as three main categories \cite{DBLP:journals/corr/abs-2201-05337}: retraining or refactoring the model, e.g. CTRL \cite{DBLP:journals/corr/abs-1909-05858}, POINTER \cite{zhang-etal-2020-pointer}, CMDP \cite{chan-etal-2021-controllable}, Constrained BART \cite{he-2021-parallel}, CoCon \cite{chan2021cocon}, PlanGen \cite{su-etal-2021-plan-generate} and InstructCTG \cite{DBLP:journals/corr/abs-2304-14293}; tuning on given data, including model fine-tuning, Prompt Tuning \cite{lester-etal-2021-power} and RL-Fine Tuning \cite{10.5555/3495724.3495977}; and post-processing, which can either design specific decoding strategy, e.g. Constrainted Beam Search \cite{anderson-etal-2017-guided}, DeLorean \cite{qin-etal-2020-back}, COLD \cite{qin2022cold}, NeuroLogic \cite{lu-etal-2021-neurologic}; or using auxilary guiding model, e.g. PPLM \cite{anderson-etal-2017-guided}, GeDI \cite{krause-etal-2021-gedi-generative}, FUDGE \cite{yang-klein-2021-fudge}, CTRLsum \cite{he-etal-2022-ctrlsum}, Plug-and-Play Content Planning \cite{liu-etal-2022-plug}, NADO \cite{meng2022controllable}, and MACSum \cite{10.1162/tacl_a_00575} .

% Conventional decoding algorithms cannot incorporate constraints during generation. Therefore, they can not ensure the output satisfies certain requirements that are important to certain applications. To this end, there exist two distinct lines of research focusing on controlled text generation which focus on constrained search algorithms and score-based sampling methods respectively. 

% Constrained search algorithms enforce strict lexical constraints on the outputs by modifying the search space according to the constraints. Constrained beam search (CBS) algorithm~\cite{anderson-etal-2017-guided}, first proposed to track constraint satisfaction using a finite-state automaton.
% However, CBS requires the model to maintain a finite-state machine with $2^C$ states (where $C$ is the number of constraints), which results in significantly increased time complexity. 
% To reduce the runtime overhead of CBS, \citet{hokamp-liu-2017-lexically} and ~\citet{post-vilar-2018-fast} introduced grid beam search (GBS) and dynamic beam allocation (DBA), respectively.
% GBS reduces inference to linear run-time complexity by grouping together hypotheses based on the number of constraints satisfied. 
% DBA further reduces the dependence on $C$ by fixing the beam size and splitting the beam into subgroups that correspond to different constraint satisfaction configurations.
% \citet{lu-etal-2021-neurologic2} introduced NeuroLogic decoding, a constrained search algorithm that aims to satisfy rich logic-based lexical constraints expressed in conjunctive normal form and extend it to NeuroLogic A$^*$ decoding~\cite{lu-etal-2022-neurologic2} by incorporating lookahead heuristics. 
% While existing constrained search algorithms significantly improve the constraint satisfaction rate, they still lead to slower generation speed and lower quality text because they prune the output distribution space aggressively and, thus, tend to collapse into globally suboptimal results. Moreover, most constrained search algorithms cannot incorporate constraint types other than lexical constraints.

% Score-based sampling methods attempt to incorporate constraints by converting constraints into differentiable score functions. Specifically, score functions for soft constraints such as sentiment control can be implemented as the cross entropy loss of corresponding classifiers. Hard constraints such as lexical constraints can be modeled by a differentiable $n$-gram matching function~\cite{liu-etal-2022-dont}. 
% With score functions that encode different constraints, controlled text generation can be achieved by score-based generative models such as Langevin dynamics based models~\cite{song2022langevin,qin2022cold,kumar2022gradient} and diffusion models~\cite{diffusion,li2022diffusionlm} on either logit space or embedding space. 
% Compared to constrained search algorithms, score-based sampling methods are more flexible because they can deal with more diverse constraint types and the composition of different constraints. However, score-based sampling methods do not come with constraint satisfaction guarantees and often lead to worse generation quality because the output distribution is modified~\cite{qin2022cold}. Moreover, score-based sampling methods lead to much slower generation speeds because multiple score-matching steps need to be performed. They also require carefully tuned relative weights between the scores of different constraints and the task-specific loss to achieve a good trade-off between the quality and the constraint satisfaction rate of output texts.

% Apart from search-based and score-based methods, \citet{dinu-etal-2019-training} proposed a similar specialized training method that appends lexical constraints to the input when training the model. Another related work is the Similarly, CTRL~\cite{keskar2019ctrl} is pre-trained with structures that naturally co-occur with raw texts and can deal with certain kinds of constraints such as style and domain constraints.\looseness=-1
% InstructCTG~\cite{zhou2023controlled} differs from these approaches because it is generally applicable to different constraint types instead of being limited to lexical constraints or constraints that can be converted into classifiers. 
% Also, instead of directly appending the constraints, as in \citet{dinu-etal-2019-training}, InstructCTG~\cite{zhou2023controlled} uses natural language instructions to verbalize, explain, and demonstrate the constraints, which makes use of the emergent abilities of large language models and helps the model generalize to unseen constraints.




==> latex/02.RelatedWork.02.tex <==
\subsection{Reinforcement Learning with Human Feedback}

Here's a merged and revised version that maintains the academic style and combines the key information from both paragraphs:

Reinforcement Learning from Human Feedback (RLHF)~\cite{bai2022rlhf, christiano2017deep, ziegler2019fine} has emerged as a crucial approach for aligning Large Language Models (LLMs) with human values and expectations, addressing the limitations of traditional supervised fine-tuning (SFT) which can lead to increased hallucinations despite improving preferred outputs. Classical RLHF algorithms, such as Proximal Policy Optimization (PPO)~\cite{schulman2017ppo}, achieve this alignment through a specialized reward model for evaluation~\cite{williams1992reinforce}, while more recent approaches like Direct Preference Optimization (DPO)~\cite{rafailov2024dpo} and its variants including SimPO~\cite{meng2024simpo}, IPO~\cite{azar2024ipo}, and KTO~\cite{ethayarajh2024kto} streamline the process by directly optimizing human preferences, thereby eliminating the need for a separate reward model and reducing computational complexity and bias~\cite{zheng2024balancing}. However, these approaches face notable challenges: RLHF generally requires substantial high-quality feedback data with detailed labeling~\cite{bai2022rlhf}, and DPO training exhibits vulnerability to overfitting, leading to poor generalization on novel data~\cite{hu2024openrlhf}, highlighting the ongoing need for improvements in model alignment techniques.

% Reinforcement Learning from Human Feedback (RLHF)~\cite{bai2022rlhf, christiano2017deep, ziegler2019fine} aims at aligning LLMs with human values and expectations.
% This approach enhances model outputs by utilizing human feedback to optimize the LLM's behavior.
% Classical RLHF algorithms, such as Proximal Policy Optimization (PPO)~\cite{schulman2017ppo} and Direct Preference Optimization (DPO)~\cite{rafailov2024dpo}, exemplify this strategy.
% PPO is widely employed due to its ability to maintain stability during training by employing a specialized reward model for evaluation~\cite{williams1992reinforce}.
% In contrast, DPO, along with its derivatives such as SimPO~\cite{meng2024simpo}, IPO~\cite{azar2024ipo}, and KTO~\cite{ethayarajh2024kto}, streamlines the process by directly optimizing human preferences, thereby eliminating the need for a separate reward model and reducing computational complexity and bias~\cite{zheng2024balancing}.
% Despite these advantages, RLHF generally demands substantial-high-quality feedback data, necessitating detailed labeling~\cite{bai2022rlhf}.
% Moreover, DPO training is prone to overfitting, resulting in poor generalization to novel data~\cite{hu2024openrlhf}.

% Supervised fine-tuning (SFT) can align models with human preferences. However, as the probability of preferred outputs increases, so does the likelihood of undesirable ones, leading to hallucinations. 
% To generate more reliable outputs, Reinforcement Learning from Human Feedback (RLHF)~\cite{ouyang2022traininglanguagemodelsfollow, christiano2017deep} has been introduced for LLM alignment. 
% This approach involves training a reward model with comparison data and then using this reward model to optimize the policy model.
% The final performance heavily depends on the quality of the reward model, and the training pipeline is quite complex.
% To simplify this process, Direct Preference Optimization (DPO)~\cite{rafailov2024dpo} was proposed, which directly uses pair-wise preference data for model optimization. This transition significantly streamlines the training pipeline. 



\subsection{Constraint Following Augmentation}

Prior work in constrained text generation can be broadly categorized into three main approaches~\cite{DBLP:journals/corr/abs-2201-05337}. 
The first category encompasses search-based methods, such as Constrained Beam Search (CBS)~\cite{anderson-etal-2017-guided} and its variants like Grid Beam Search (GBS)~\cite{hokamp-liu-2017-lexically} and Dynamic Beam Allocation (DBA)~\cite{post-vilar-2018-fast}, which enforce lexical constraints by modifying the search space, though often at the cost of generation speed and quality. The second category consists of score-based sampling methods that transform constraints into differentiable score functions~\cite{liu-etal-2022-dont}, offering greater flexibility in handling diverse constraint types but lacking guaranteed constraint satisfaction and suffering from slower generation speeds~\cite{qin2022cold}. The third category focuses on model-centric approaches, including specialized training methods and large language models like CTRL~\cite{keskar2019ctrl} and InstructCTG~\cite{DBLP:journals/corr/abs-2304-14293}, which incorporate constraints through pre-training or natural language instructions. Recent advancements have explored multiple directions: multi-attribute controlled text generation through prefix tuning~\cite{li2021prefix}; latent space manipulation techniques such as MacLaSa~\cite{ding-etal-2023-maclasa} and MAGIC~\cite{liu-etal-2024-multi}, where the latter employs counterfactual feature vectors to disentangle attributes; regular expression-based constraint generation through REI~\cite{zheng2023toward}; and the development of specialized datasets~\cite{zhang-etal-2023-macsum} to improve control ability while maintaining text quality.

==> latex/05.Experiment.01.tex <==


\subsection{Overall Result}

实验分析主要写：

各个指标下GAPO效果很好

在什么场合下，指标不一致

在什么case下，


\input{tabs/tab_IFEval}

\input{tabs/tab_PDD}

\subsection{Training Efficiency}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/plot.png}
    \caption{在不同训练方法下，模型的训练量和效果之间的关系}
    \label{fig:training_plot}
\end{figure}

\subsection{Result on Different Prompt Difficulties}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/detail.png}
    \caption{GAPO的表现和什么因素相关}
    \label{fig:detail_performance}
\end{figure*}


\subsection{Details in Adversarial Process}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/adversarial.png}
    \caption{对抗阶段的具体表现}
    \label{fig:adversarial}
\end{figure}

\subsection{Case Study}
xxx



==> latex/08.App.MoreExperiments.01.tex <==


\input{tabs/tab_PDD_app}
\input{tabs/tab_IFEVAL_app}

==> old_version/01.Introduction.01.tex <==

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/intro.png}
    \caption{Caption}
    \label{fig:intro}
\end{figure}

Ensuring that language models can handle constraints during text generation is crucial. 
One effective approach to this is to control constraints at the data level. 
Data-level control can generally be achieved through two main types of synthetic data generation. 
The first type directly synthesizes instruction-response pairs that satisfy the constraints, providing clear examples of compliant responses. 
The second type, which is often more effective, uses preference data to adjust the probability distribution, enhancing the likelihood that the model outputs a correct response over an incorrect one.

The first approach, although useful, often leads to ``hallucination'' problems, where the model generates content that diverges from the intended constraints. 
This limitation makes the second method—preference-based data synthesis—more widely used. 
A straightforward way to achieve preference-based data synthesis is to create pairs where prompts have been deliberately altered to produce responses that are either aligned or misaligned with constraints, providing the model with comparative examples. 
This method is simple, easy to implement, and supports fine-grained contrastive learning between correct and incorrect responses.

While this straightforward method offers utility, it often struggles to address more complex constraints, especially in decoder-only models. 
Due to their unidirectional attention mechanism, decoder-only models have difficulty recognizing mismatches between prompt and response. 
To enable more accurate understanding, we propose using an encoder-only model. 
With its bidirectional attention, an encoder-only model is well-suited to comprehending two-way dependencies in text and can more effectively discern inappropriate prompts for specific responses.

To refine this process further, we utilize Proximal Policy Optimization~(PPO), which efficiently uses rewards from the encoder-only model’s discriminator to train the generator. 
The encoder-only model acts as a discriminator, assessing response compliance with constraints. 
Additionally, we employ a Generative Adversarial Network~(GAN) to enhance this setup. 
In the GAN framework, the generator produces responses while the discriminator iteratively strengthens its ability to identify constraint violations by leveraging feedback from the generator’s current outputs. 
This iterative “enhancement” of the discriminator is essential, as it progressively sharpens the model’s capacity to detect nuanced violations, leading to more reliable constraint-aware responses.




==> old_version/03.Method.05.tex <==
\subsection{Preliminary of Constrained Generation}

The process of constraint generation can be described as follows. Given an input prompt \( P = (\mathcal{T}, \mathcal{C}) \), where \( \mathcal{T} \) represents a free-text description and \( \mathcal{C} = \{C_1, C_2, \dots, C_n\} \) is a set of constraints, the objective is to generate an output \( R \) that satisfies all constraints in \( \mathcal{C} \). This can be formulated as an expectation maximization problem:
\[
E(\pi_\theta) = \mathbb{E}_{R \sim \pi_\theta(P)} \left[ \sum_{C_i \in \mathcal{C}} \mathcal{L}(R, C_i) \right], \tag{1} \label{eq:expectation_maximization}
\]
where \( \pi_\theta(P) \) denotes the generative model parameterized by \( \theta \), producing outputs \( R \) given \( P \). The function \( \mathcal{L}(R, C_i) \) measures the satisfaction of constraint \( C_i \) by the generated output \( R \). Typically, \( \mathcal{L}(R, C_i) \) is defined as a binary indicator:
\[
\mathcal{L}(R, C_i) =
\begin{cases} 
1 & \text{if } R \models C_i, \\
0 & \text{otherwise.}
\end{cases} \tag{2} \label{eq:binary_loss}
\]

\begin{table}[t]
\centering
\caption{Symbol Definitions}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lp{0.9\columnwidth}}
\toprule
\textbf{Symbol} & \textbf{Definition} \\
\midrule
\( \mathcal{T} \) & Free-text description in a prompt \\
\( \mathcal{C} \) & Set of constraints \\
\( P \) & Input prompt \( (\mathcal{T}, \mathcal{C}) \) \\
\( R \) & Generated output, or say the response of a Generator \\
\( \pi_\theta \) & Generative model parameterized by \( \theta \) \\
\( \mathcal{L}(R, C_i) \) & Constraint satisfaction function \\
\( \mathcal{D} \) & Original dataset \\
\( \mathcal{D}' \) & Augmented dataset \\
\( R(s, a) \) & Reward model output for state-action pair \\
\( \pi_\text{ref} \) & Reference generator distribution \\
\( V^\pi(s) \) & Critic model value function for state \( s \) \\
\( Q^\pi(s, a) \) & Cumulative reward for state-action pair \\
\( r_t(\theta) \) & Probability ratio between generator and \newline reference generator \\
\( A_t \) & Advantage function for action \( a \) in \newline state \( s \) \\
\bottomrule
\end{tabular}}
\label{tab:symbol_definitions}
\end{table}

\subsection{Constraint-Aware Data Augmentation for Preference Learning}

To facilitate preference learning, we propose a method for constraint-aware data augmentation. The dataset is represented as \( \mathcal{D} = \{(P_i, R_i)\}_{i=1}^N \), where \( P_i = (\mathcal{T}_i, \mathcal{C}_i) \) consists of a free-text description and a set of constraints. For each \( P_i \), two types of prompts are created: an accept prompt, which satisfies the original constraints \( \mathcal{C}_i \), and a reject prompt, where the constraints \( \mathcal{C}_i \) are modified to form \( \mathcal{C}_i^{\text{reject}} \), ensuring that at least one constraint is unsatisfiable. The augmented dataset is then expressed as:
\[
\mathcal{D}' = \{(P_i^{\text{accept}}, R_i), (P_i^{\text{reject}}, R_i)\}_{i=1}^N, \tag{3} \label{eq:augmented_dataset}
\]
where \( P_i^{\text{reject}} = (\mathcal{T}_i, \mathcal{C}_i^{\text{reject}}) \) and \( \mathcal{C}_i^{\text{reject}} \) satisfies:
\[
\exists C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}}, \quad \mathcal{L}(R_i, C_{i,j}^{\text{reject}}) = 0. \tag{4} \label{eq:reject_condition}
\]

The accept and reject prompts share the same free-text description \( \mathcal{T}_i \) and response \( R_i \), allowing the model to distinguish between valid and invalid constraints during training.

\subsection{Adversarial Training Framework}

To improve constraint-aware text generation, an adversarial training framework is employed. This framework consists of several key components, including a generator \( \pi_\theta(a|s) \), a reference generator \( \pi_\text{ref}(a|s) \), a reward model \( R(s, a) \), and a critic model \( V^\pi(s) \). 

The reward model is trained using the augmented dataset \( \mathcal{D}' \), which is extended to include accept prompts, reject prompts, and original prompts paired with either human-written or generated responses. This dataset is represented as:
\begin{align}
\mathcal{D}' = \big\{ & (P_i^{\text{accept}}, R_i, y=1), \nonumber\\
                      & (P_i^{\text{reject}}, R_i, y=0), \tag{5} \label{eq:reward_dataset} \\
                      & (P_i, \hat{R}_i, y=0) \big\}. \nonumber
\end{align}
where \( y \) denotes whether the response is acceptable or not. The reward model minimizes the binary cross-entropy loss:
\begin{align}
L_R(\theta) = - &\mathbb{E}_{(s, a, y) \sim \mathcal{D}'} \big[  y \log R(s, a) \tag{6} \label{eq:reward_loss} \\
    & + (1 - y) \log \left( 1 - R(s, a) \right) \big]. \nonumber
\end{align}
where \( \theta \) represents the model parameters.

The generator \( \pi_\theta \) is optimized using Proximal Policy Optimization (PPO) to balance reward maximization and proximity to the reference generator \( \pi_\text{ref} \). The objective is expressed as:
\[
L_{\text{G}}(\theta) = \mathbb{E}_t \left[ r_t(\theta) A_t \right], \tag{7} \label{eq:ppo_loss}
\]
where the probability ratio \( r_t(\theta) \) is defined as:
\[
r_t(\theta) = \frac{\pi_\theta(a_t|s_t)}{\pi_\text{ref}(a_t|s_t)}, \tag{8} \label{eq:ratio}
\]
and the advantage function \( A_t \) quantifies the difference between the cumulative reward \( Q^\pi(s_t, a_t) \) and the baseline value \( V^\pi(s_t) \):
\[
A_t = Q^\pi(s_t, a_t) - V^\pi(s_t). \tag{9} \label{eq:advantage}
\]
The cumulative reward \( Q^\pi(s_t, a_t) \) is computed as:
\[
Q^\pi(s_t, a_t) = R(s_t, a_t) + \gamma \mathbb{E}_{s_{t+1} \sim \pi_\theta}[V^\pi(s_{t+1})]. \tag{10} \label{eq:q_function}
\]
During adversarial training, the Generator $\pi_\theta$ aims to maximize the Reward Model's evaluations. It is updated using PPO with the objective:
\begin{align}
L_{\text{G}}(\theta) = \mathbb{E}_{(s_t, a_t) \sim \pi_\theta} \Big[ & \min \big( r_t(\theta) A_t, \tag{11} \label{eq:ppo_loss} \\
    & \text{clip} \big( r_t(\theta), 1 - \epsilon, 1 + \epsilon \big) A_t \big) \Big]. \nonumber
\end{align}




The Critic Model $V^\pi(s)$ estimates expected rewards and is updated by minimizing:
\[
L_C(\theta) = \mathbb{E}_{s} \left[ \left( V^\pi(s) - R(s, a) \right)^2 \right], \tag{12} \label{eq:critic_loss}
\]
where $\theta$ denotes its parameters.






==> old_version/03.Method.06.tex <==
\subsection{Preliminary of Constrained Generation}

Let us formally define the constrained generation problem. 
Given an input prompt $P = (\mathcal{T}, \mathcal{C})$, where $\mathcal{T}$ denotes a free-text description and $\mathcal{C} = \{C_1, C_2, \dots, C_n\}$ represents a set of constraints, our objective is to generate an output $R$ that satisfies all constraints in $\mathcal{C}$. We formulate this as an expectation maximization problem:
\[
E(\pi_\theta) = \mathbb{E}_{R \sim \pi_\theta(P)} \left[ \sum_{C_i \in \mathcal{C}} \mathcal{L}(R, C_i) \right], \tag{1}
\]
where $\pi_\theta(P)$ represents the generative model parameterized by $\theta$. The constraint satisfaction function $\mathcal{L}(R, C_i)$ is defined as:
\[
\mathcal{L}(R, C_i) =
\begin{cases} 
1 & \text{if } R \models C_i, \\
0 & \text{otherwise.}
\end{cases} \tag{2}
\]

\begin{table}[t]
\centering
\caption{Notation and Definitions}
\begin{tabular}{ll}
\toprule
\textbf{Symbol} & \textbf{Definition} \\
\midrule
$\mathcal{T}$ & Free-text description component \\
$\mathcal{C}$ & Constraint set \\
$P$ & Input prompt $(\mathcal{T}, \mathcal{C})$ \\
$R$ & Generated output \\
$\pi_\theta(a|c)$ & Generative model with parameters $\theta$ \\
$\mathcal{L}(R, C_i)$ & Constraint satisfaction function \\
$\mathcal{D}$ & Training dataset \\
$\mathcal{D}'$ & Augmented dataset \\
$R(s, a)$ & Reward function \\
$V^\pi(s)$ & Value function \\
$Q^\pi(s, a)$ & Action-value function \\
\bottomrule
\end{tabular}
\label{tab:notation}
\end{table}

\subsection{Constraint-Aware Data Augmentation}

We propose a data augmentation method for constraint-aware learning. 
Given a dataset $\mathcal{D} = \{(P_i, R_i)\}_{i=1}^N$, where each prompt $P_i = (\mathcal{T}_i, \mathcal{C}_i)$, we construct an augmented dataset through constraint perturbation. For each original constraint set $\mathcal{C}_i$, we generate a rejected constraint set $\mathcal{C}_i^{\text{reject}}$ through one of the following operations:

1) \textbf{Constraint Modification}: For a randomly selected constraint $C_{i,j} \in \mathcal{C}_i$, we modify it to create $C_{i,j}^{\text{reject}}$ such that it becomes incompatible with the original response $R_i$:
\[
C_{i,j}^{\text{reject}} = f_{\text{modify}}(C_{i,j}), \quad \text{where} \quad \mathcal{L}(R_i, C_{i,j}^{\text{reject}}) = 0
\]

2) \textbf{Constraint Insertion}: We introduce an additional constraint $C_{i,n+1}^{\text{reject}}$ that conflicts with existing constraints:
\[
\mathcal{C}_i^{\text{reject}} = \mathcal{C}_i \cup \{C_{i,n+1}^{\text{reject}}\}, \quad \text{where} \quad \mathcal{L}(R_i, C_{i,n+1}^{\text{reject}}) = 0
\]

The augmented dataset is thus constructed as:
\[
\mathcal{D}' = \{(P_i^{\text{accept}}, R_i), (P_i^{\text{reject}}, R_i)\}_{i=1}^N, \tag{3}
\]
where $P_i^{\text{accept}} = (\mathcal{T}_i, \mathcal{C}_i)$ and $P_i^{\text{reject}} = (\mathcal{T}_i, \mathcal{C}_i^{\text{reject}})$. This augmentation strategy ensures that:
\[
\exists C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}}: \mathcal{L}(R_i, C_{i,j}^{\text{reject}}) = 0. \tag{4}
\]

% Through this process, we create a balanced dataset containing both satisfiable and unsatisfiable constraint sets, while maintaining the semantic relationship between the text description $\mathcal{T}_i$ and the response $R_i$. This augmented dataset enables the model to learn the distinction between valid and invalid constraints effectively.

\subsection{Adversarial Learning Framework}

We propose an adversarial learning framework comprising a generator $\pi_\theta(a|s)$, a reward model $R(s, a)$, and a value function $V^\pi(s)$. The reward model is trained on the augmented dataset:
\begin{align}
\mathcal{D}' = \big\{ & (P_i^{\text{accept}}, R_i, 1), \nonumber\\
                      & (P_i^{\text{reject}}, R_i, 0), \tag{5} \\
                      & (P_i, \hat{R}_i, 0) \big\}. \nonumber
\end{align}
, where $\hat{R}_i$ represents the response generated by the generator based on prompt $P_i$.
And the reward model optimizes the cross-entropy loss:
\[
L_R(\theta) = -\mathbb{E}_{(s, a, y) \sim \mathcal{D}'} \left[ y \log R(s, a) + (1 - y) \log(1 - R(s, a)) \right]. \tag{6}
\]

The generator's objective function is formulated as:
\[
L_G(\theta) = \mathbb{E}_t \left[ \frac{\pi_\theta(a_t|s_t)}{\pi_{\text{ref}}(a_t|s_t)} A_t \right], \tag{7}
\]
where the advantage function $A_t$ is defined as:
\[
A_t = Q^\pi(s_t, a_t) - V^\pi(s_t), \tag{8}
\]
and the action-value function is:
\[
Q^\pi(s_t, a_t) = R(s_t, a_t) + \gamma \mathbb{E}_{s_{t+1} \sim \pi_\theta}[V^\pi(s_{t+1})]. \tag{9}
\]

The value function is optimized by minimizing the mean squared error:
\[
L_V(\theta) = \mathbb{E}_{s} \left[ \left(V^\pi(s) - R(s, a)\right)^2 \right]. \tag{10}
\]

==> old_version/03.Preliminary.01.tex <==
% \subsection{Reinforcement Learning with Proximal Policy Optimization (PPO)}

% PPO算法是一种广泛应用的强化学习优化方法，其目标是通过约束策略更新幅度，确保训练过程稳定。给定策略 $\pi_\theta(a|s)$，其优化目标为：
% \[
% L^{\text{PPO}}(\theta) = \mathbb{E}_t \left[ \min(r_t(\theta) A_t, \text{clip}(r_t(\theta), 1 - \epsilon, 1 + \epsilon) A_t) \right],
% \]
% 其中 $r_t(\theta) = \frac{\pi_\theta(a_t|s_t)}{\pi_{\theta_\text{old}}(a_t|s_t)}$ 为策略概率比，$A_t$ 为优势函数，$\epsilon$ 为超参数。

% \subsection{Generative Adversarial Networks (GAN)}

% GAN由生成器（Generator）和判别器（Discriminator）组成。生成器试图生成以假乱真的数据，而判别器的目标是区分真实数据和生成数据。其目标函数定义为：
% \[
% \min_G \max_D \mathbb{E}_{x \sim p_\text{data}(x)}[\log D(x)] + \mathbb{E}_{z \sim p_z(z)}[\log (1 - D(G(z)))].
% \]

\subsection{Reinforcement Learning with Proximal Policy Optimization (PPO)}

PPO通过对策略更新的约束，实现语言模型生成分布的稳定优化，依赖生成器、参考生成器、奖励模型和评论员模型的协作。

\subsubsection*{模型建模}

- \textbf{生成器 ($\pi_\theta$)}：语言模型，定义为 $\pi_\theta(a|s)$，在上下文 $s$ (Context) 下生成下一个Token $a$ (Next Token) 的概率分布，是优化目标。

- \textbf{参考生成器 ($\pi_\text{ref}$)}：固定或缓慢更新的参考语言模型 $\pi_\text{ref}(a|s)$，限制生成器的分布与其不偏离过远。

- \textbf{奖励模型 ($R(s, a)$)}：评估生成文本质量的评分函数，通常基于人工标注的偏好数据或任务指标训练。

- \textbf{评论员模型 ($V^\pi(s)$)}：估计上下文 $s$ (Context) 的值函数，作为基线减少生成策略更新的方差。

\subsubsection*{优化目标}

PPO的优化目标为调整生成器 $\pi_\theta$ 的行为分布，使其获得更高奖励，同时限制与参考生成器 $\pi_\text{ref}$ 的偏差。其优化目标公式为：
\[
L^{\text{PPO}}(\theta) = \mathbb{E}_t \left[ r_t(\theta) A_t \right],
\]
其中 $r_t(\theta)$ 是当前策略与参考策略的概率比：
\[
r_t(\theta) = \frac{\pi_\theta(a_t|s_t)}{\pi_\text{ref}(a_t|s_t)},
\]
而 $A_t$ 是优势函数，计算公式为：
\[
A_t = Q^\pi(s_t, a_t) - V^\pi(s_t),
\]
其中 $Q^\pi(s_t, a_t)$ 是生成器从状态 $s_t$ 生成 $a_t$ 后的累计奖励：
\[
Q^\pi(s_t, a_t) = R(s_t, a_t) + \gamma \mathbb{E}_{s_{t+1} \sim \pi_\theta}[V^\pi(s_{t+1})].
\]

\subsubsection*{训练过程}

1. 使用生成器 $\pi_\theta$ 基于上下文 (Context) 采样生成下一个Token (Next Token)，并计算生成概率 $\pi_\theta(a|s)$。
2. 通过奖励模型 $R(s, a)$ 对生成文本进行评分，结合评论员模型 $V^\pi(s)$ 估计状态值，计算优势函数 $A_t$。
3. 使用 $L^{\text{PPO}}(\theta)$ 优化生成器 $\pi_\theta$，使生成策略逐步向高奖励区域收敛。
4. 定期更新参考生成器 $\pi_\text{ref}$ 以适应当前策略。

\subsection{Generative Adversarial Networks (GAN)}

GAN通过生成器与奖励模型的对抗训练生成高质量文本。在文本生成任务中，由于离散生成的特性，生成器的优化依赖强化学习框架。为了提升对生成过程的监督效果，额外引入了Rollout判别模型和Hyper判别模型。

\subsubsection*{模型建模}

- \textbf{生成器 ($G_\theta$)}：语言生成模型，定义为 $G_\theta(a|s)$，基于上下文 $s$ (Context) 生成下一个Token $a$ (Next Token)。目标是使生成文本的分布接近真实数据分布。

- \textbf{奖励模型 ($R$)}：提供生成样本的全局奖励，用于评估文本的整体质量。

- \textbf{Rollout判别模型 ($D_R$)}：在生成中间步骤评估部分序列的质量，提供短期监督信号。模型通过未完成序列的隐状态预测其成为高质量文本的可能性，从而指导生成器优化中间生成步骤。

- \textbf{Hyper判别模型 ($D_H$)}：在生成结束后，判断生成文本是否满足全局目标，例如是否符合上下文约束或质量要求。该模型提供长远奖励，用于校正生成器的整体方向。

\subsubsection*{优化目标}

GAN的整体目标是通过生成器与双重判别模型的对抗训练优化生成策略：
\[
\min_{G_\theta} \max_{D_R, D_H} \mathbb{E}_{x \sim p_{\text{data}}(x)} \left[ \log D_H(x) \right] + \mathbb{E}_{z \sim p_z(z)} \left[ \log (1 - D_H(G_\theta(a|s))) \right].
\]

同时，为了缓解生成中间步骤与最终奖励之间的偏差，使用Monte Carlo采样估计未完成序列的奖励，定义行动-值函数 $Q_G$ 为：
\[
Q_G(a_t, Y_{1:t-1}, s_0) =
\begin{cases} 
\frac{1}{N} \sum_{n=1}^N D_R(s_0, Y_{1:t-1}^n), & t < T, \\
D_H(Y_{1:T}, s_0), & t = T,
\end{cases}
\]
其中 $Y_{1:t-1}$ 表示部分序列，$T$ 为生成完成时的长度，$N$ 为采样次数。

\subsubsection*{监督作用}

- \textbf{Rollout判别模型的监督}：Rollout判别模型 $D_R$ 为每个中间生成步骤提供奖励估计，减少生成过程中稀疏奖励的问题。它采用轻量化的模型（如LSTM）对部分序列进行隐状态计算，得到生成质量的短期评估。

- \textbf{Hyper判别模型的监督}：Hyper判别模型 $D_H$ 在生成完成后提供全局评估信号，判断生成文本是否符合目标分布。通过结合上下文嵌入和生成文本表示，进一步细化长远监督。

通过双重判别模型，GAN能够在生成过程中有效捕捉文本质量信息，平衡短期和长期奖励，从而提升生成文本的质量与一致性。


==> old_version/03.Preliminary.02.tex <==
\subsection{Reinforcement Learning with Proximal Policy Optimization (PPO)}

Proximal Policy Optimization (PPO) stabilizes the optimization of the language model's generative distribution by coordinating four components: 
The \textbf{Generator} ($\pi_\theta$), defined as $\pi_\theta(a|s)$, is the primary language model generating the probability distribution for the next token $a$ given context $s$ and serves as the main optimization target. The \textbf{Reference Generator} ($\pi_\text{ref}$), represented by $\pi_\text{ref}(a|s)$, is fixed or updated periodically to constrain the generator and prevent divergence from a baseline distribution. 
The \textbf{Reward Model} ($R(s, a)$) evaluates text quality through a scoring function trained on preference data or task-specific metrics. 
Finally, the \textbf{Critic Model} ($V^\pi(s)$) estimates the value of a context $s$, providing a baseline to reduce variance in policy updates.


The optimization goal in PPO is to adjust the generator $\pi_\theta$ to maximize rewards while maintaining proximity to the reference generator $\pi_\text{ref}$. The objective is defined as:
\[
L^{\text{PPO}}(\theta) = \mathbb{E}_t \left[ r_t(\theta) A_t \right],
\]
where $r_t(\theta)$ is the ratio of probabilities between the generator and reference generator:
\[
r_t(\theta) = \frac{\pi_\theta(a_t|s_t)}{\pi_\text{ref}(a_t|s_t)}.
\]
The advantage function $A_t$ quantifies the benefit of a specific action compared to the critic model's baseline:
\[
A_t = Q^\pi(s_t, a_t) - V^\pi(s_t),
\]
where $Q^\pi(s_t, a_t)$ is the cumulative reward for taking action $a_t$ in state $s_t$:
\[
Q^\pi(s_t, a_t) = R(s_t, a_t) + \gamma \mathbb{E}_{s_{t+1} \sim \pi_\theta}[V^\pi(s_{t+1})].
\]

\subsection{Generative Adversarial Networks (GAN)}

Generative Adversarial Networks (GANs) improve text generation quality through adversarial training, involving the generator, reward model, and critic model. The generator $G_\theta(a|s)$, given context $s$, generates the probability of the next token $a$ and seeks to approximate the real data distribution. The reward model $R(s, a)$ provides global feedback by evaluating the overall quality of generated sequences. The critic model $V^\pi(s)$ estimates the quality of partially generated sequences, offering short-term feedback to guide intermediate steps of generation.



GANs optimize the generator by minimizing a loss function that integrates feedback from both the reward model and intermediate sequence evaluations. The generator seeks to maximize the reward for generated sequences while improving intermediate outputs. The generator's loss function is defined as:
\[
L_{G} = -\mathbb{E}_{Y \sim G_\theta} \left[ R(Y) \right],
\]
where $R(Y)$ is the reward model's evaluation of the full generated sequence $Y$.

For intermediate supervision, the action-value function $Q_G$ provides estimated rewards for partial sequences using Monte Carlo sampling:
\[
Q_G(a_t, Y_{1:t-1}) =
\begin{cases} 
\frac{1}{N} \sum_{n=1}^N R(Y_{1:t-1}^n), & t < T, \\
R(Y_{1:T}), & t = T,
\end{cases}
\]
where $Y_{1:t-1}$ is the partial sequence at step $t$, $T$ is the total sequence length, and $N$ is the number of sampled rollouts.

The generator is updated to maximize $Q_G$ at each step of generation. The reinforcement learning policy gradient method adjusts the generator's parameters $\theta$ based on:
\[
\nabla_\theta L_{G} = -\mathbb{E}_{Y \sim G_\theta} \left[ \nabla_\theta \log G_\theta(a|s) Q_G(a, Y_{1:t-1}) \right],
\]
where $G_\theta(a|s)$ represents the generator's probability of selecting action $a$ given context $s$. This loss function effectively combines intermediate feedback and final rewards, ensuring coherent and high-quality text generation.


\subsection{Constraint Generation}

The \textbf{Constraint Generation} is modeled as follows: Given an input prompt \( P = (\mathcal{T}, \mathcal{C}) \), where \( \mathcal{T} \) is a free-text description and \( \mathcal{C} = \{C_1, C_2, \dots, C_n\} \) is a set of constraints, the goal is to generate an output \( R \) such that all constraints in \( \mathcal{C} \) are satisfied. This can be expressed as an expectation maximization problem:
\[
E(\pi_\theta) = \mathbb{E}_{R \sim \pi_\theta(P)} \left[ \sum_{C_i \in \mathcal{C}} \mathcal{L}(R, C_i) \right],
\]
where:
\( \pi_\theta(P) \) is the generative model parameterized by \( \theta \), producing outputs \( R \) given \( P \).
\( \mathcal{L}(R, C_i) \) measures the satisfaction of constraint \( C_i \) by the generated output \( R \), often defined as a binary indicator (\( \mathcal{L} = 1 \) if \( R \models C_i \), \( 0 \) otherwise) or a graded reward.


==> old_version/03.Preliminary.03.tex <==
\subsection{Constraint Generation}

The \textbf{Constraint Generation} is modeled as follows: Given an input prompt \( P = (\mathcal{T}, \mathcal{C}) \), where \( \mathcal{T} \) is a free-text description and \( \mathcal{C} = \{C_1, C_2, \dots, C_n\} \) is a set of constraints, the goal is to generate an output \( R \) such that all constraints in \( \mathcal{C} \) are satisfied. This can be expressed as an expectation maximization problem:
\[
E(\pi_\theta) = \mathbb{E}_{R \sim \pi_\theta(P)} \left[ \sum_{C_i \in \mathcal{C}} \mathcal{L}(R, C_i) \right],
\]
where:
\( \pi_\theta(P) \) is the generative model parameterized by \( \theta \), producing outputs \( R \) given \( P \).
\( \mathcal{L}(R, C_i) \) measures the satisfaction of constraint \( C_i \) by the generated output \( R \), often defined as a binary indicator (\( \mathcal{L} = 1 \) if \( R \models C_i \), \( 0 \) otherwise) or a graded reward.


==> old_version/03.Preliminary.04.tex <==
\subsection{Constraint Generation}

The process of constraint generation can be described as follows. Given an input prompt \( P = (\mathcal{T}, \mathcal{C}) \), where \( \mathcal{T} \) represents a free-text description and \( \mathcal{C} = \{C_1, C_2, \dots, C_n\} \) is a set of constraints, the objective is to generate an output \( R \) that satisfies all constraints in \( \mathcal{C} \). This can be formulated as an expectation maximization problem:
\[
E(\pi_\theta) = \mathbb{E}_{R \sim \pi_\theta(P)} \left[ \sum_{C_i \in \mathcal{C}} \mathcal{L}(R, C_i) \right], \tag{1} \label{eq:expectation_maximization}
\]
where \( \pi_\theta(P) \) denotes the generative model parameterized by \( \theta \), producing outputs \( R \) given \( P \). The function \( \mathcal{L}(R, C_i) \) measures the satisfaction of constraint \( C_i \) by the generated output \( R \). Typically, \( \mathcal{L}(R, C_i) \) is defined as a binary indicator:
\[
\mathcal{L}(R, C_i) =
\begin{cases} 
1 & \text{if } R \models C_i, \\
0 & \text{otherwise.}
\end{cases} \tag{2} \label{eq:binary_loss}
\]


==> old_version/04.Method.01.tex <==
\subsection{Data Augmentation for Constraint-Aware Preference Data Pair}

我们设计了一种约束感知的数据增强方法，以生成适合偏好学习的配对数据（Preference Data Pair）。以下将形式化地定义和描述这一过程。

设训练数据为 $\mathcal{D} = \{(p_i, r_i)\}_{i=1}^N$，其中 $p_i$ 为Prompt，$r_i$ 为对应的真实响应（Response）。我们通过引入约束条件的变体，生成以下两类增强数据：
1. **Accept Prompt**: 满足约束条件的Prompt，记为 $p_i^{\text{accept}}$。
2. **Reject Prompt**: 不满足约束条件的Prompt，记为 $p_i^{\text{reject}}$。

构建的数据对为：
\[
\mathcal{D}' = \{(p_i^{\text{accept}}, r_i), (p_i^{\text{reject}}, r_i)\}_{i=1}^N.
\]

具体而言，约束感知的数据增强包含以下步骤：
1. 对每个Prompt $p_i$ 进行修改，引入条件偏差 $\delta$，使得：
   \[
   p_i^{\text{accept}} = p_i + \delta^{\text{accept}}, \quad p_i^{\text{reject}} = p_i + \delta^{\text{reject}},
   \]
   其中 $\delta^{\text{accept}}$ 和 $\delta^{\text{reject}}$ 分别表示正向和负向的约束修正。
2. 生成增强数据对 $\{(p_i^{\text{accept}}, r_i), (p_i^{\text{reject}}, r_i)\}$，用于训练模型在不同约束下的响应偏好。

通过上述数据增强，我们能够为生成器提供更多的训练信号，帮助其学习对不同Prompt的偏好关系。

---

\subsection{GANPPO}

基于增强后的数据集，我们提出了GANPPO（Generative Adversarial Network with PPO），一种对抗性学习算法，用于优化语言生成模型的性能。GANPPO的核心思想是结合奖励模型、判别器（Critic Model）和生成器，通过联合优化提升生成质量。

\subsubsection{Objective of Reward Model}

奖励模型 $D$ 的目标是区分真实响应和生成器生成的响应。基于数据增强构造的配对数据 $(p_i^{\text{accept}}, r_i)$ 和 $(p_i^{\text{reject}}, r_i)$，奖励模型的优化目标为：
\[
L_D = -\mathbb{E}_{(p, r) \sim \mathcal{D}'} \left[ \log D(p, r) \right] - \mathbb{E}_{(p, r_g) \sim \mathcal{G}} \left[ \log (1 - D(p, r_g)) \right],
\]
其中：
- $D(p, r)$ 为奖励模型对数据 $(p, r)$ 的评分；
- $\mathcal{G}$ 表示生成器生成的数据分布。

通过优化 $L_D$，奖励模型学习如何有效区分生成器生成的响应和真实响应。

\subsubsection{Objective of Critic Model}

Critic模型 $C$ 的目标是学习Prompt与部分响应之间的关系。其目标函数为：
\[
L_C = -\mathbb{E}_{(p, r_{\text{partial}}) \sim \mathcal{D}'} \left[ \log C(p, r_{\text{partial}}) \right] - \mathbb{E}_{(p, r_{\text{gen-partial}}) \sim \mathcal{G}} \left[ \log (1 - C(p, r_{\text{gen-partial}})) \right],
\]
其中 $r_{\text{partial}}$ 表示部分真实响应，$r_{\text{gen-partial}}$ 表示生成的部分响应。

\subsubsection{Objective of Generator}

生成器 $G$ 的目标是基于Prompt $p$ 生成高质量的响应 $r_g$，使其能够获得高奖励值 $R(p, r_g)$。生成器的优化目标为：
\[
L_G = -\mathbb{E}_{p \sim \mathcal{P}} \left[ R(p, r_g) \right],
\]
其中 $R(p, r_g)$ 由奖励模型 $D$ 的评分提供，具体为 $R(p, r_g) = D(p, r_g)$。

此外，为保证生成响应的多样性和语义一致性，我们引入基于PPO的正则化项，最终目标函数为：
\[
L_G^{\text{PPO}} = -\mathbb{E}_{p \sim \mathcal{P}} \left[ R(p, r_g) - \alpha \cdot \text{KL}(\pi_\theta || \pi_{\text{ref}}) \right],
\]
其中：
- $\alpha$ 为正则化系数；
- $\text{KL}(\pi_\theta || \pi_{\text{ref}})$ 表示生成器与参考策略的KL散度。

\subsubsection{Training Procedure}

GANPPO的训练分为两个阶段：

1. **Cold Start Phase:** 使用数据增强方法预训练生成器和奖励模型，初始化生成器的基本能力。
2. **Adversarial Training Phase:** 生成器与奖励模型通过对抗训练交替优化。

完整训练伪代码如下：

\begin{algorithm}
\caption{GANPPO Training Procedure}
\begin{algorithmic}[1]
\REQUIRE Training dataset $\mathcal{D}$, generator $G$, reward model $D$, critic model $C$
\STATE Initialize $G$, $D$, $C$, and their optimizers
\FOR{epoch in $1, \dots, N$}
    \STATE Sample $(p, r)$ from $\mathcal{D}$ and generate $r_g$ using $G$
    \STATE Update $D$ using loss $L_D$
    \STATE Update $C$ using loss $L_C$
    \STATE Update $G$ using loss $L_G^{\text{PPO}}$
\ENDFOR
\end{algorithmic}
\label{alg:ganppo}
\end{algorithm}


==> old_version/04.Method.02.tex <==
% \subsection{Constraint-Aware Data Augmentation for Preference Learning}


% To generate preference data pairs for training, we introduce a constraint-aware augmentation method. 
% Let the original dataset be \( \mathcal{D} = \{(P_i, R_i)\}_{i=1}^N \), where \( P_i = (\mathcal{T}_i, \mathcal{C}_i) \) denotes a prompt as define in Eq.\ref{}.
% For each prompt \( P_i \), we define two types of augmented data:
% \textbf{Accept Prompt} (\( P_i^{\text{accept}} \)): A prompt where the constraints \( \mathcal{C}_i \) remain valid.
% \textbf{Reject Prompt} (\( P_i^{\text{reject}} \)): A prompt derived by systematically altering \( \mathcal{C}_i \) to create \( \mathcal{C}_i^{\text{reject}} \), where at least one \( C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}} \) is unsatisfiable.

% The augmented dataset is then expressed as:
% \[
% \mathcal{D}' = \{(P_i^{\text{accept}}, R_i), (P_i^{\text{reject}}, R_i)\}_{i=1}^N.
% \]

% Specifically, the reject prompt \( P_i^{\text{reject}} \) is constructed as:
% \[
% P_i^{\text{reject}} = (\mathcal{T}_i, \mathcal{C}_i^{\text{reject}}),
% \]
% where \( \mathcal{C}_i^{\text{reject}} \) is obtained by introducing deliberate violations to one or more constraints in \( \mathcal{C}_i \), ensuring:
% \[
% \exists C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}}, \quad \mathcal{L}(R_i, C_{i,j}^{\text{reject}}) = 0.
% \]

% This approach ensures that \( P_i^{\text{accept}} \) and \( P_i^{\text{reject}} \) are directly comparable, as they share the same free-text description \( \mathcal{T}_i \) and response \( R_i \). By training on such paired data, the model learns to distinguish between prompts that satisfy all constraints and those that do not.


\subsection{Constraint-Aware Data Augmentation for Preference Learning}

We propose a constraint-aware augmentation method to generate preference data pairs. Given the dataset \( \mathcal{D} = \{(P_i, R_i)\}_{i=1}^N \), where \( P_i = (\mathcal{T}_i, \mathcal{C}_i) \) as defined in Eq.\ref{}, we construct two types of prompts for each \( P_i \):
\textbf{Accept Prompt} (\( P_i^{\text{accept}} \)): Satisfies the original constraints \( \mathcal{C}_i \).
\textbf{Reject Prompt} (\( P_i^{\text{reject}} \)): Modifies \( \mathcal{C}_i \) to create \( \mathcal{C}_i^{\text{reject}} \), where at least one \( C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}} \) is unsatisfiable.


The augmented dataset is:
\[
\mathcal{D}' = \{(P_i^{\text{accept}}, R_i), (P_i^{\text{reject}}, R_i)\}_{i=1}^N,
\]
where \( P_i^{\text{reject}} = (\mathcal{T}_i, \mathcal{C}_i^{\text{reject}}) \) and \( \mathcal{C}_i^{\text{reject}} \) is designed such that:
\[
\exists C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}}, \quad \mathcal{L}(R_i, C_{i,j}^{\text{reject}}) = 0.
\]

This ensures \( P_i^{\text{accept}} \) and \( P_i^{\text{reject}} \) share the same free-text description \( \mathcal{T}_i \) and response \( R_i \), enabling the model to learn distinctions between valid and invalid constraints. 


\subsection{Adversarial Training Framework}

We develop an adversarial training framework that integrates Proximal Policy Optimization (PPO) with Generative Adversarial Networks (GAN) to enhance constraint-aware text generation. The core components are the \textbf{Generator} $\pi_\theta(a|s)$, the \textbf{Reward Model} $R(s, a)$, and the \textbf{Critic Model} $V^\pi(s)$.

Initially, the Reward Model $R(s, a)$ is trained as a classifier using the augmented dataset $\mathcal{D}'$:
\[
\mathcal{D}' = \left\{ (P_i^{\text{accept}}, R_i, y=1),\ (P_i^{\text{reject}}, R_i, y=0),\ (P_i, \hat{R}_i, y=0) \right\},
\]
where:
$P_i^{\text{accept}}$ is the accept prompt.
$P_i^{\text{reject}}$ is the reject prompt with unsatisfiable constraints.
$P_i$ is the original prompt.
$R_i$ is the human-written response.
$\hat{R}_i$ is the response generated by the Generator.
$y$ is the label indicating acceptable ($y=1$) or unacceptable ($y=0$) responses.

The Reward Model minimizes the binary cross-entropy loss:
\[
L_R(\phi) = - \mathbb{E}_{(s, a, y) \sim \mathcal{D}'} \left[ y \log R(s, a) + (1 - y) \log \left( 1 - R(s, a) \right) \right],
\]
with $\phi$ representing its parameters.

During adversarial training, the Generator $\pi_\theta$ aims to maximize the Reward Model's evaluations. It is updated using PPO with the objective:

\[
L^{\text{PPO}}(\theta) = \mathbb{E}_{(s_t, a_t) \sim \pi_\theta} \left[ \min \left( r_t(\theta) A_t,\ \text{clip} \left( r_t(\theta),\ 1 - \epsilon,\ 1 + \epsilon \right) A_t \right) \right],
\]

where:
$r_t(\theta) = \dfrac{\pi_\theta(a_t | s_t)}{\pi_{\text{ref}}(a_t | s_t)}$ is the probability ratio.
$\epsilon$ is a clipping hyperparameter.
The advantage function is $A_t = R(s_t, a_t) - V^\pi(s_t)$.

The Critic Model $V^\pi(s)$ estimates expected rewards and is updated by minimizing:
\[
L_V(\psi) = \mathbb{E}_{s} \left[ \left( V^\pi(s) - R(s, a) \right)^2 \right],
\]
where $\psi$ denotes its parameters.

The joint optimization objectives are:
\[
\min_{\theta} -L^{\text{PPO}}(\theta), \quad \min_{\phi} L_R(\phi), \quad \min_{\psi} L_V(\psi).
\]
This framework ensures the Generator produces responses satisfying the constraints (accepted by $R(s, a)$), while the Reward Model and Critic Model continuously refine their evaluations.

==> old_version/04.Method.03.tex <==

\subsection{Constraint-Aware Data Augmentation for Preference Learning}

We propose a constraint-aware augmentation method to generate preference data pairs. Given the dataset \( \mathcal{D} = \{(P_i, R_i)\}_{i=1}^N \), where \( P_i = (\mathcal{T}_i, \mathcal{C}_i) \) as defined in Eq.\ref{}, we construct two types of prompts for each \( P_i \):
\textbf{Accept Prompt} (\( P_i^{\text{accept}} \)): Satisfies the original constraints \( \mathcal{C}_i \).
\textbf{Reject Prompt} (\( P_i^{\text{reject}} \)): Modifies \( \mathcal{C}_i \) to create \( \mathcal{C}_i^{\text{reject}} \), where at least one \( C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}} \) is unsatisfiable.


The augmented dataset is:
\[
\mathcal{D}' = \{(P_i^{\text{accept}}, R_i), (P_i^{\text{reject}}, R_i)\}_{i=1}^N,
\]
where \( P_i^{\text{reject}} = (\mathcal{T}_i, \mathcal{C}_i^{\text{reject}}) \) and \( \mathcal{C}_i^{\text{reject}} \) is designed such that:
\[
\exists C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}}, \quad \mathcal{L}(R_i, C_{i,j}^{\text{reject}}) = 0.
\]

This ensures \( P_i^{\text{accept}} \) and \( P_i^{\text{reject}} \) share the same free-text description \( \mathcal{T}_i \) and response \( R_i \), enabling the model to learn distinctions between valid and invalid constraints. 


\subsection{Adversarial Training Framework}

We develop an adversarial training framework that integrates Proximal Policy Optimization (PPO) with Generative Adversarial Networks (GAN) to enhance constraint-aware text generation. The core components are the \textbf{Generator} $\pi_\theta(a|s)$, the \textbf{Reference Generator}  $\pi_\text{ref}(a|s)$, the \textbf{Reward Model} $R(s, a)$, and the \textbf{Critic Model} $V^\pi(s)$. 


Initially, the Reward Model $R(s, a)$ is trained as a classifier using the augmented dataset $\mathcal{D}'$:
\[
\mathcal{D}' = \left\{ (P_i^{\text{accept}}, R_i, y=1),\ (P_i^{\text{reject}}, R_i, y=0),\ (P_i, \hat{R}_i, y=0) \right\},
\]
where:
$P_i^{\text{accept}}$ is the accept prompt.
$P_i^{\text{reject}}$ is the reject prompt with unsatisfiable constraints.
$P_i$ is the original prompt.
$R_i$ is the human-written response.
$\hat{R}_i$ is the response generated by the Generator.
$y$ is the label indicating acceptable ($y=1$) or unacceptable ($y=0$) responses.

The Reward Model minimizes the binary cross-entropy loss:
\[
L_R(\phi) = - \mathbb{E}_{(s, a, y) \sim \mathcal{D}'} \left[ y \log R(s, a) + (1 - y) \log \left( 1 - R(s, a) \right) \right],
\]
with $\phi$ representing its parameters.

To adjust the generator $\pi_\theta$ to maximize rewards while maintaining proximity to the reference generator $\pi_\text{ref}$. The objective is defined as:
\[
L^{\text{PPO}}(\theta) = \mathbb{E}_t \left[ r_t(\theta) A_t \right],
\]
where $r_t(\theta)$ is the ratio of probabilities between the generator and reference generator:
\[
r_t(\theta) = \frac{\pi_\theta(a_t|s_t)}{\pi_\text{ref}(a_t|s_t)}.
\]
The advantage function $A_t$ quantifies the benefit of a specific action compared to the critic model's baseline:
\[
A_t = Q^\pi(s_t, a_t) - V^\pi(s_t),
\]
where $Q^\pi(s_t, a_t)$ is the cumulative reward for taking action $a_t$ in state $s_t$:
\[
Q^\pi(s_t, a_t) = R(s_t, a_t) + \gamma \mathbb{E}_{s_{t+1} \sim \pi_\theta}[V^\pi(s_{t+1})].
\]



==> old_version/04.Method.04.tex <==
\begin{table}[t]
\centering
\caption{Symbol Definitions}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lp{0.9\columnwidth}}
\toprule
\textbf{Symbol} & \textbf{Definition} \\
\midrule
\( \mathcal{T} \) & Free-text description in a prompt \\
\( \mathcal{C} \) & Set of constraints \\
\( P \) & Input prompt \( (\mathcal{T}, \mathcal{C}) \) \\
\( R \) & Generated output, or say the response of a Generator \\
\( \pi_\theta \) & Generative model parameterized by \( \theta \) \\
\( \mathcal{L}(R, C_i) \) & Constraint satisfaction function \\
\( \mathcal{D} \) & Original dataset \\
\( \mathcal{D}' \) & Augmented dataset \\
\( R(s, a) \) & Reward model output for state-action pair \\
\( \pi_\text{ref} \) & Reference generator distribution \\
\( V^\pi(s) \) & Critic model value function for state \( s \) \\
\( Q^\pi(s, a) \) & Cumulative reward for state-action pair \\
\( r_t(\theta) \) & Probability ratio between generator and \newline reference generator \\
\( A_t \) & Advantage function for action \( a \) in \newline state \( s \) \\
\bottomrule
\end{tabular}}
\label{tab:symbol_definitions}
\end{table}

\subsection{Constraint-Aware Data Augmentation for Preference Learning}

To facilitate preference learning, we propose a method for constraint-aware data augmentation. The dataset is represented as \( \mathcal{D} = \{(P_i, R_i)\}_{i=1}^N \), where \( P_i = (\mathcal{T}_i, \mathcal{C}_i) \) consists of a free-text description and a set of constraints. For each \( P_i \), two types of prompts are created: an accept prompt, which satisfies the original constraints \( \mathcal{C}_i \), and a reject prompt, where the constraints \( \mathcal{C}_i \) are modified to form \( \mathcal{C}_i^{\text{reject}} \), ensuring that at least one constraint is unsatisfiable. The augmented dataset is then expressed as:
\[
\mathcal{D}' = \{(P_i^{\text{accept}}, R_i), (P_i^{\text{reject}}, R_i)\}_{i=1}^N, \tag{3} \label{eq:augmented_dataset}
\]
where \( P_i^{\text{reject}} = (\mathcal{T}_i, \mathcal{C}_i^{\text{reject}}) \) and \( \mathcal{C}_i^{\text{reject}} \) satisfies:
\[
\exists C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}}, \quad \mathcal{L}(R_i, C_{i,j}^{\text{reject}}) = 0. \tag{4} \label{eq:reject_condition}
\]

The accept and reject prompts share the same free-text description \( \mathcal{T}_i \) and response \( R_i \), allowing the model to distinguish between valid and invalid constraints during training.

\subsection{Adversarial Training Framework}

To improve constraint-aware text generation, an adversarial training framework is employed. This framework consists of several key components, including a generator \( \pi_\theta(a|s) \), a reference generator \( \pi_\text{ref}(a|s) \), a reward model \( R(s, a) \), and a critic model \( V^\pi(s) \). 

The reward model is trained using the augmented dataset \( \mathcal{D}' \), which is extended to include accept prompts, reject prompts, and original prompts paired with either human-written or generated responses. This dataset is represented as:
\begin{align}
\mathcal{D}' = \big\{ & (P_i^{\text{accept}}, R_i, y=1), \nonumber\\
                      & (P_i^{\text{reject}}, R_i, y=0), \tag{5} \label{eq:reward_dataset} \\
                      & (P_i, \hat{R}_i, y=0) \big\}. \nonumber
\end{align}
where \( y \) denotes whether the response is acceptable or not. The reward model minimizes the binary cross-entropy loss:
\begin{align}
L_R(\theta) = - &\mathbb{E}_{(s, a, y) \sim \mathcal{D}'} \big[  y \log R(s, a) \tag{6} \label{eq:reward_loss} \\
    & + (1 - y) \log \left( 1 - R(s, a) \right) \big]. \nonumber
\end{align}
where \( \theta \) represents the model parameters.

The generator \( \pi_\theta \) is optimized using Proximal Policy Optimization (PPO) to balance reward maximization and proximity to the reference generator \( \pi_\text{ref} \). The objective is expressed as:
\[
L_{\text{G}}(\theta) = \mathbb{E}_t \left[ r_t(\theta) A_t \right], \tag{7} \label{eq:ppo_loss}
\]
where the probability ratio \( r_t(\theta) \) is defined as:
\[
r_t(\theta) = \frac{\pi_\theta(a_t|s_t)}{\pi_\text{ref}(a_t|s_t)}, \tag{8} \label{eq:ratio}
\]
and the advantage function \( A_t \) quantifies the difference between the cumulative reward \( Q^\pi(s_t, a_t) \) and the baseline value \( V^\pi(s_t) \):
\[
A_t = Q^\pi(s_t, a_t) - V^\pi(s_t). \tag{9} \label{eq:advantage}
\]
The cumulative reward \( Q^\pi(s_t, a_t) \) is computed as:
\[
Q^\pi(s_t, a_t) = R(s_t, a_t) + \gamma \mathbb{E}_{s_{t+1} \sim \pi_\theta}[V^\pi(s_{t+1})]. \tag{10} \label{eq:q_function}
\]
During adversarial training, the Generator $\pi_\theta$ aims to maximize the Reward Model's evaluations. It is updated using PPO with the objective:
\begin{align}
L_{\text{G}}(\theta) = \mathbb{E}_{(s_t, a_t) \sim \pi_\theta} \Big[ & \min \big( r_t(\theta) A_t, \tag{11} \label{eq:ppo_loss} \\
    & \text{clip} \big( r_t(\theta), 1 - \epsilon, 1 + \epsilon \big) A_t \big) \Big]. \nonumber
\end{align}




The Critic Model $V^\pi(s)$ estimates expected rewards and is updated by minimizing:
\[
L_C(\theta) = \mathbb{E}_{s} \left[ \left( V^\pi(s) - R(s, a) \right)^2 \right], \tag{12} \label{eq:critic_loss}
\]
where $\theta$ denotes its parameters.






==> old_version/05.ExperimentSetup.01.tex <==



% \subsection{Experiment Setup}

% \subsubsection{Dataset}

% \subsubsection{Baselines}

% \textbf{Models}

% Qwen


% \textbf{Augmentation Methods}


% \subsection{Overall Experiment}

% \subsection{对抗细节}

% Reward Model 和 其他评估方法 随着Generator的提升
% - x轴是Generator的训练step数
% - y轴是打分
% - 每个颜色的线表示一种打分方法

% 训练开销

% \subsection{xxxx}

% 训练开销一览

% \subsection{xxx}

% \subsection{Case Study}


\subsection{Baselines}
The experiments conducted primarily encompass two types of role-playing methods outlined as follows.

\subsubsection{Prompt Based Method}
\textbf{(1) Direct Ask:} This method directly probes the model's personality without role-playing instructions to evaluate inherent biases.
\textbf{(2) Direct Role-Playing:} The model is explicitly instructed on the role it is expected to play and assumes this role without additional prompts.
\textbf{(3) Contextual Role-Playing:} This approach briefs the model on the role and requires it to generate relevant role-specific information, including personality traits, to inform its role-playing.

\subsubsection{Fine-tune Based Method}
\textbf{(4) Supervised Fine-Tuning~(SFT):} The model is fine-tuned with a role-playing-specific dataset to enhance its performance in role-playing scenarios.
\textbf{(5) DPO:}~\cite{rafailov2024direct} DPO tries to increase the likelihood of generating annotated accept data while lowering the probability of rejecting data.
\textbf{(6) KTO:}~\cite{ethayarajh2024kto} KTO applies prospect theory to maximize the utility of outputs directly, outperforming preference-based methods with binary feedback.
\textbf{(7) SimPO:}~\cite{meng2024simpo} SimPO simplifies preference optimization by aligning the reward function with model generation and eliminating the need for a reference model.
\textbf{(8) Step-DPO:}~\cite{lai2024step} Step-DPO improves long-chain reasoning by optimizing individual reasoning steps rather than full answers. 
\textbf{(9) Multi-DPO:} Multi-DPO equally differentiates among all preference categories.
\textbf{(10) DMPO~(Ours):} DMPO optimizes similar preference data in similar directions, enhancing the model by utilizing the inherent similarities among preferences.

\subsection{Training Dataset}
We primarily conducted our experiments using datasets from nine roles within the Character-LLM Dataset~\cite{shao2023character}.
To mitigate the potential loss of generalizability~\cite{zhou2024lima,gu2024xiezhi} associated with using only domain-specific data, we supplemented our data with ShareGPT~\cite{sharegpt} and CodeGPT~\cite{codegpt} datasets.

Since dialog data cannot be directly used for DPO training, we enhanced it using the method proposed in this paper.
We assumed the Character-LLM data to be "RF \& IF" data and synthesized approximately equal amounts of "Non RF \& IF," "RF \& Non IF," and "Non RF \& Non IF" data.
During the generation of "Non RF \& IF" data, we utilized Qwen2-72B-chat for an auxiliary generation.

Detailed statistics of each dataset and the quantity of data used in our experiments are provided in Table~\ref{tab:dataset_details_2}.


\subsection{Models}
\textbf{GPT-4o:} This model exhibits advanced capabilities in contextual comprehension and response generation, making it particularly suitable for dynamic interactive applications.
\textbf{GLM-4:} It produces coherent long-text responses, enhancing narrative consistency.
\textbf{QWen2-7B-Instruct~(Qwen2-7B):} Designed for executing complex instructions, this model demonstrates high accuracy in task-oriented dialogues.
\textbf{Chatglm3-6b-chat~(ChatGLM3-6B):} Optimized for chat applications, this model effectively balances conversational dynamics with the provision of informative content.
\textbf{Mistral-7b-chat~(Mistral-7B):} Excelling in chat-based scenarios, this model is adept at handling nuanced dialogues and maintaining conversational context.


\subsection{Evaluation}
This module assesses Role-Play LLMs' proficiency in embodying character-specific personality traits using the InCharacter~\cite{wang2023incharacter} framework.

\subsubsection{Test Suite:}
We mainly use two test suites in InCharacter to test baselines that can be directly used based on the Naive Training Dataset in Tab.~\ref{tab:baseline_result}.
Moreover, use all InCharacter datasets to test fine-tuning methods based on Enhanced Dataset in Tab.~\ref{tab:tune_result}:
\textbf{Myers-Briggs Type Indicator~(MBTI)}~\cite{rutinowski2024self, pan2023llms}: Analyzes psychological preferences in perception and decision-making, categorizing personalities into 16 types.
\textbf{Big Five Personality Indicator~(BFI)}~\cite{bodroza2023personality, serapio2023personality, romero2023gpt}: Describes personality through five broad dimensions (OCEAN), predicting behavioral patterns and various life outcomes.
Here is the revised version in English:

\subsubsection{Metrics:}
 \textbf{Accuracy per Dimension} (\texttt{Acc$_\text{Dim}$}): Measures the precision of Role-Play LLMs' responses within specific personality dimensions.
 \textbf{Full Accuracy} (\texttt{Acc$_\text{Full}$}): Indicates the overall accuracy of RPAs across all personality dimensions.
 \textbf{Mean Absolute Error} (\texttt{MAE}): Quantifies the average error magnitude in Role-Play LLMs' personality assessments.
 \textbf{Standard Deviation of Dimension} (\texttt{Std$_\text{Dim}$}): Evaluates the variability in Role-Play LLMs' responses to individual personality test items.
 \textbf{Standard Deviation across Dimensions} (\texttt{Std$_\text{Full}$}): Assesses the consistency of Role-Play LLMs' portrayals across different personality dimensions.
 \textbf{Standard Deviation of Scores} (\texttt{Std$_\text{MAE}$}): Measures the overall stability of Role-Play LLMs' personality scores throughout the testing phase.



==> old_version/cc.tex <==
\section{Preliminary}

\subsection{Reinforcement Learning with Proximal Policy Optimization (PPO)}

Proximal Policy Optimization (PPO) stabilizes the optimization of the language model's generative distribution by coordinating four components: 
The \textbf{Generator} ($\pi_\theta$), defined as $\pi_\theta(a|s)$, is the primary language model generating the probability distribution for the next token $a$ given context $s$ and serves as the main optimization target. The \textbf{Reference Generator} ($\pi_\text{ref}$), represented by $\pi_\text{ref}(a|s)$, is fixed or updated periodically to constrain the generator and prevent divergence from a baseline distribution. 
The \textbf{Reward Model} ($R(s, a)$) evaluates text quality through a scoring function trained on preference data or task-specific metrics. 
Finally, the \textbf{Critic Model} ($V^\pi(s)$) estimates the value of a context $s$, providing a baseline to reduce variance in policy updates.


The optimization goal in PPO is to adjust the generator $\pi_\theta$ to maximize rewards while maintaining proximity to the reference generator $\pi_\text{ref}$. The objective is defined as:
\[
L^{\text{PPO}}(\theta) = \mathbb{E}_t \left[ r_t(\theta) A_t \right],
\]
where $r_t(\theta)$ is the ratio of probabilities between the generator and reference generator:
\[
r_t(\theta) = \frac{\pi_\theta(a_t|s_t)}{\pi_\text{ref}(a_t|s_t)}.
\]
The advantage function $A_t$ quantifies the benefit of a specific action compared to the critic model's baseline:
\[
A_t = Q^\pi(s_t, a_t) - V^\pi(s_t),
\]
where $Q^\pi(s_t, a_t)$ is the cumulative reward for taking action $a_t$ in state $s_t$:
\[
Q^\pi(s_t, a_t) = R(s_t, a_t) + \gamma \mathbb{E}_{s_{t+1} \sim \pi_\theta}[V^\pi(s_{t+1})].
\]

\subsection{Generative Adversarial Networks (GAN)}

Generative Adversarial Networks (GANs) improve text generation quality through adversarial training, involving the generator, reward model, and critic model. The generator $G_\theta(a|s)$, given context $s$, generates the probability of the next token $a$ and seeks to approximate the real data distribution. The reward model $R(s, a)$ provides global feedback by evaluating the overall quality of generated sequences. The critic model $V^\pi(s)$ estimates the quality of partially generated sequences, offering short-term feedback to guide intermediate steps of generation.



GANs optimize the generator by minimizing a loss function that integrates feedback from both the reward model and intermediate sequence evaluations. The generator seeks to maximize the reward for generated sequences while improving intermediate outputs. The generator's loss function is defined as:
\[
L_{G} = -\mathbb{E}_{Y \sim G_\theta} \left[ R(Y) \right],
\]
where $R(Y)$ is the reward model's evaluation of the full generated sequence $Y$.

For intermediate supervision, the action-value function $Q_G$ provides estimated rewards for partial sequences using Monte Carlo sampling:
\[
Q_G(a_t, Y_{1:t-1}) =
\begin{cases} 
\frac{1}{N} \sum_{n=1}^N R(Y_{1:t-1}^n), & t < T, \\
R(Y_{1:T}), & t = T,
\end{cases}
\]
where $Y_{1:t-1}$ is the partial sequence at step $t$, $T$ is the total sequence length, and $N$ is the number of sampled rollouts.

The generator is updated to maximize $Q_G$ at each step of generation. The reinforcement learning policy gradient method adjusts the generator's parameters $\theta$ based on:
\[
\nabla_\theta L_{G} = -\mathbb{E}_{Y \sim G_\theta} \left[ \nabla_\theta \log G_\theta(a|s) Q_G(a, Y_{1:t-1}) \right],
\]
where $G_\theta(a|s)$ represents the generator's probability of selecting action $a$ given context $s$. This loss function effectively combines intermediate feedback and final rewards, ensuring coherent and high-quality text generation.


\subsection{Constraint Generation}

The \textbf{Constraint Generation} is modeled as follows: Given an input prompt \( P = (\mathcal{T}, \mathcal{C}) \), where \( \mathcal{T} \) is a free-text description and \( \mathcal{C} = \{C_1, C_2, \dots, C_n\} \) is a set of constraints, the goal is to generate an output \( R \) such that all constraints in \( \mathcal{C} \) are satisfied. This can be expressed as an expectation maximization problem:
\[
E(\pi_\theta) = \mathbb{E}_{R \sim \pi_\theta(P)} \left[ \sum_{C_i \in \mathcal{C}} \mathcal{L}(R, C_i) \right],
\]
where:
\( \pi_\theta(P) \) is the generative model parameterized by \( \theta \), producing outputs \( R \) given \( P \).
\( \mathcal{L}(R, C_i) \) measures the satisfaction of constraint \( C_i \) by the generated output \( R \), often defined as a binary indicator (\( \mathcal{L} = 1 \) if \( R \models C_i \), \( 0 \) otherwise) or a graded reward.


\section{Method}


\subsection{Constraint-Aware Data Augmentation for Preference Learning}

We propose a constraint-aware augmentation method to generate preference data pairs. Given the dataset \( \mathcal{D} = \{(P_i, R_i)\}_{i=1}^N \), where \( P_i = (\mathcal{T}_i, \mathcal{C}_i) \) as defined in Eq.\ref{}, we construct two types of prompts for each \( P_i \):
\textbf{Accept Prompt} (\( P_i^{\text{accept}} \)): Satisfies the original constraints \( \mathcal{C}_i \).
\textbf{Reject Prompt} (\( P_i^{\text{reject}} \)): Modifies \( \mathcal{C}_i \) to create \( \mathcal{C}_i^{\text{reject}} \), where at least one \( C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}} \) is unsatisfiable.


The augmented dataset is:
\[
\mathcal{D}' = \{(P_i^{\text{accept}}, R_i), (P_i^{\text{reject}}, R_i)\}_{i=1}^N,
\]
where \( P_i^{\text{reject}} = (\mathcal{T}_i, \mathcal{C}_i^{\text{reject}}) \) and \( \mathcal{C}_i^{\text{reject}} \) is designed such that:
\[
\exists C_{i,j}^{\text{reject}} \in \mathcal{C}_i^{\text{reject}}, \quad \mathcal{L}(R_i, C_{i,j}^{\text{reject}}) = 0.
\]

This ensures \( P_i^{\text{accept}} \) and \( P_i^{\text{reject}} \) share the same free-text description \( \mathcal{T}_i \) and response \( R_i \), enabling the model to learn distinctions between valid and invalid constraints. 


\subsection{Adversarial Training Framework}

We develop an adversarial training framework that integrates Proximal Policy Optimization (PPO) with Generative Adversarial Networks (GAN) to enhance constraint-aware text generation. The core components are the \textbf{Generator} $\pi_\theta(a|s)$, the \textbf{Reward Model} $R(s, a)$, and the \textbf{Critic Model} $V^\pi(s)$.

Initially, the Reward Model $R(s, a)$ is trained as a classifier using the augmented dataset $\mathcal{D}'$:
\[
\mathcal{D}' = \left\{ (P_i^{\text{accept}}, R_i, y=1),\ (P_i^{\text{reject}}, R_i, y=0),\ (P_i, \hat{R}_i, y=0) \right\},
\]
where:
$P_i^{\text{accept}}$ is the accept prompt.
$P_i^{\text{reject}}$ is the reject prompt with unsatisfiable constraints.
$P_i$ is the original prompt.
$R_i$ is the human-written response.
$\hat{R}_i$ is the response generated by the Generator.
$y$ is the label indicating acceptable ($y=1$) or unacceptable ($y=0$) responses.

The Reward Model minimizes the binary cross-entropy loss:
\[
L_R(\phi) = - \mathbb{E}_{(s, a, y) \sim \mathcal{D}'} \left[ y \log R(s, a) + (1 - y) \log \left( 1 - R(s, a) \right) \right],
\]
with $\phi$ representing its parameters.

During adversarial training, the Generator $\pi_\theta$ aims to maximize the Reward Model's evaluations. It is updated using PPO with the objective:

\[
L^{\text{PPO}}(\theta) = \mathbb{E}_{(s_t, a_t) \sim \pi_\theta} \left[ \min \left( r_t(\theta) A_t,\ \text{clip} \left( r_t(\theta),\ 1 - \epsilon,\ 1 + \epsilon \right) A_t \right) \right],
\]

where:
$r_t(\theta) = \dfrac{\pi_\theta(a_t | s_t)}{\pi_{\text{ref}}(a_t | s_t)}$ is the probability ratio.
$\epsilon$ is a clipping hyperparameter.
The advantage function is $A_t = R(s_t, a_t) - V^\pi(s_t)$.

The Critic Model $V^\pi(s)$ estimates expected rewards and is updated by minimizing:
\[
L_V(\psi) = \mathbb{E}_{s} \left[ \left( V^\pi(s) - R(s, a) \right)^2 \right],
\]
where $\psi$ denotes its parameters.

The joint optimization objectives are:
\[
\min_{\theta} -L^{\text{PPO}}(\theta), \quad \min_{\phi} L_R(\phi), \quad \min_{\psi} L_V(\psi).
\]
This framework ensures the Generator produces responses satisfying the constraints (accepted by $R(s, a)$), while the Reward Model and Critic Model continuously refine their evaluations.



==> tabs/tab_IFEVAL_app.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccccccc}
\toprule
\textbf{Model} & \textbf{Prompt} & \textbf{Punctuation} & \textbf{Format} & \textbf{Length} & \textbf{Content} & \textbf{Combination} & \textbf{ChangeCase} & \textbf{Startend} & \textbf{Keywords} & \textbf{Language} & \textbf{All} \\
\midrule
Llama-3.1-7B & \texttt{Naive Prompt} & - & - & - & - & - & - & - & - & - & - \\
Llama-3.1-7B & \texttt{CoT Prompt} & - & - & - & - & - & - & - & - & - & - \\
Llama-3.1-7B & \texttt{Plan-N-Solve Prompt} & - & - & - & - & - & - & - & - & - & - \\
\midrule
Llama-3.1-7B + \textbf{SFT} & \texttt{Naive Prompt} & - & - & - & - & - & - & - & - & - & - \\
Llama-3.1-7B + \textbf{DPO} & \texttt{Naive Prompt} & - & - & - & - & - & - & - & - & - & - \\
Llama-3.1-7B + \textbf{KTO} & \texttt{Naive Prompt} & - & - & - & - & - & - & - & - & - & - \\
Llama-3.1-7B + \textbf{SimPO} & \texttt{Naive Prompt} & - & - & - & - & - & - & - & - & - & - \\
% Llama-3.1-7B + \textbf{PRM} & \texttt{Naive Prompt} & - & - & - & - & - & - & - & - & - & - \\
Llama-3.1-7B + \textbf{ORPO} & \texttt{Naive Prompt} & - & - & - & - & - & - & - & - & - & - \\
Llama-3.1-7B + \textbf{PPO} & \texttt{Naive Prompt} & - & - & - & - & - & - & - & - & - & - \\
Llama-3.1-7B + \textbf{GAPO} & \texttt{Naive Prompt} & - & - & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}}
\caption{Performance Comparison Across Different Categories}
\label{tab:ifeval_app}
\end{table*}

==> tabs/tab_PDD_app.tex <==

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llccccccc}
\toprule
\multirow{3}{*}{\textbf{Model}} & \multirow{3}{*}{\textbf{Prompt}} & \multicolumn{3}{c}{\textbf{Reward Model}} & \multicolumn{2}{c}{\textbf{LLM-as-a-Judge}} & \multirow{3}{*}{\textbf{Human}} & \multirow{3}{*}{\textbf{Overall}} \\
\cline{3-7}
\multicolumn{2}{c}{} & \textbf{\begin{tabular}[c]{@{}c@{}}Roberta-\\Small-4096\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Roberta-\\Base-4096\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Roberta-\\Large-4096\end{tabular}} & \textbf{GPT-4o} & \textbf{GPT3.5-turbo} & \multicolumn{2}{c}{} \\
\midrule
Llama-3.1-7B & \texttt{Naive Prompt} & - & 0.556 & - & - & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{Comprehensive Model Performance Comparison}
\label{tab:pdd_app}
\end{table*}

==> tabs/tab_pp_pr.tex <==

\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{l|llc|llc}
    \toprule
        \textbf{Model} & \textbf{\#Sample} & \textbf{\#Token} & \textbf{PDD Perfromance} & \textbf{\#Sample} & \textbf{\#Token} & \textbf{IFEval Performance}\\
        \addlinespace[1pt]
        \hline
        \rowcolor{gray!25}
        \multicolumn{7}{l}{
        \textbf{\textit{No Training}}} \\
        \hline
        \addlinespace[1pt]
        Qwen-2.5-7B & - & - & 61.4 & - & - & 52.3 \\
        \addlinespace[1pt]
        \hline
        \rowcolor{gray!25}
        \multicolumn{7}{l}{
        \textbf{\textit{No Preferential Data}}} \\ 
        \hline
        \addlinespace[1pt]
        Qwen-2.5-7B + \textbf{SFT} & 3,300 & 6,561,531 & 70.1 & 432 & 687,810 & - \\
        \addlinespace[1pt]
        \hline
        \rowcolor{gray!25}
        \multicolumn{7}{l}{
        \textbf{\textit{Training w/ Preferential Response}}} \\
        \hline
        \addlinespace[1pt]
        Qwen-2.5-7B + \textbf{PPO} & 2,000 & 4,295,575 & 65.8 & 400 & 613,842 & - \\
        Qwen-2.5-7B + \textbf{PPO} & 4,000 & 8,660,218 & 72.4 & 600 & 925,910 & - \\
        Qwen-2.5-7B + \textbf{PPO} & 6,600 & 13,243,796 & 78.5 & 864 & 1,230,481 & - \\
        Qwen-2.5-7B + \textbf{GAPO} & 2,000 & 4,295,575 & 70.3 & 400 & 613,842 & - \\
        Qwen-2.5-7B + \textbf{GAPO} & 4,000 & 8,660,218 & 76.4 & 600 & 925,910 & - \\
        Qwen-2.5-7B + \textbf{GAPO} & 6,600 & 13,243,796 & 82.9 & 864 & 1,230,481 & - \\
        \addlinespace[1pt]
        \hline
        \rowcolor{gray!25}
        \multicolumn{7}{l}{
        \textbf{\textit{Training w/ Preferential Prompt}}} \\
        \hline
        \addlinespace[1pt]
        Qwen-2.5-7B + \textbf{PPO} & 2,000 & 4,219,814 & 68.5 & 400 & 610,916 & - \\
        Qwen-2.5-7B + \textbf{PPO} & 4,000 & 8,506,194 & 75.1 & 600 & 924,572 & - \\
        Qwen-2.5-7B + \textbf{PPO} & 6,600 & 12,984,601 & 89.4 & 864 & 1,223,975 & - \\
        Qwen-2.5-7B + \textbf{GAPO} & 2,000 & 4,219,814 & 70.6 & 400 & 610,916 & - \\
        Qwen-2.5-7B + \textbf{GAPO} & 4,000 & 8,506,194 & 81.3 & 600 & 924,572 & - \\
        Qwen-2.5-7B + \textbf{GAPO} & 6,600 & 12,984,601 & 95.4 & 864 & 1,223,975 & - \\
        \bottomrule
    \end{tabular}
    \caption{Comparative Analysis of using Preferential Response and Preferential Prompt.
The PDD Performance metric represents the model's generative output on the PDD dataset, as evaluated using a fine-tuned LongFormer-Large-4096 Reward model architecture.
The IFEval Performance metric indicates the model's comprehensive performance across the IFEval benchmark framework.}
    \label{tab:pp_pr_old}
\end{table*}
